Winner's bliss: interdependent-value auctions with horizontal uncertainty

We analyze auctions with interdependent values and horizontally differentiated bidders, where good news for one bidder is bad news for the other bidders. This generates a winner's bliss, reversing the well-known winner's curse: winning means buying an object that is more valuable than a na\"{\i}ve estimate suggests. Our main result is about the English auction. We introduce the ``own effect property,'' generalizing the single-crossing condition, to prove the existence of an efficient ex-post equilibrium. Regarding revenue, we show that with affiliated signals, the English auction yields no more revenue than the second-price auction, while independent signals yield the standard revenue equivalence.

==> Figures/Comparison.tex <==

\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        axis lines = left,
        xlabel = {$\mathbf{x}$},
        ylabel = {$p$},
        legend pos=north west,
        domain=0:1, % Restrict the domain to [0, 1]
        samples=100,
        ymin=0.5, ymax=2.5, % Adjust the y-axis to fit the new functions
        xtick={0,1}, % Only label 0 and 1 on the x-axis
        xticklabels={$\mathbf{0}$, $\mathbf{1}$}, % Set the labels to bold
        ytick={1,2}, % Remove all y-axis tick labels
        yticklabels={$\underline{p}$, $\bar{p}$},
    ]
    
    % First function: \sigma(x) = x^2 + 1
    \addplot[thick, blue] {x^2 + 1};
    \addlegendentry{$\sigma^{-1}(\mathbf{x})$}

    % Second function: \sigma'(x) = x^4 + 1
    \addplot[thick, red, dashed] {x^4 + 1};
    \addlegendentry{$\sigma'^{-1}(\mathbf{x})$}
    
    \end{axis}
\end{tikzpicture}
    \caption{An Example illustrates the relationship between the price $p$ and the $\sigma$ function}
    \label{fig:compare}
\end{figure}





